Methods and Techniques for Dynamic Deployability of Software-Defined Security Services

With the recent trend of "network softwarisation", enabled by emerging technologies such as Software-Defined Networking (SDN) and Network Function Virtualisation (NFV), system administrators of data centres and enterprise networks have started replacing dedicated hardware-based middleboxes with virtualised network functions running on servers and end hosts. This radical change has facilitated the provisioning of advanced and flexible network services, ultimately helping system administrators and network operators to cope with the rapid changes in service requirements and networking workloads. This thesis investigates the challenges of provisioning network security services in "softwarised" networks, where the security of residential and business users can be provided by means of sets of software-based network functions running on high performance servers or on commodity compute devices. The study is approached from the perspective of the telecom operator, whose goal is to protect the customers from network threats and, at the same time, maximize the number of provisioned services, and thereby revenue. Specifically, the overall aim of the research presented in this thesis is proposing novel techniques for optimising the resource usage of software-based security services, hence for increasing the chances for the operator to accommodate more service requests while respecting the desired level of network security of its customers. In this direction, the contributions of this thesis are the following: (i) a solution for the dynamic provisioning of security services that minimises the utilisation of computing and network resources, and (ii) novel methods based on Deep Learning and Linux kernel technologies for reducing the CPU usage of software-based security network functions, with specific focus on the defence against Distributed Denial of Service (DDoS) attacks.

==> application-centric-security/acronyms.tex <==
% Use them with \ac{acronym name}, \acp{acronym name} for plurals, \acl{acronym name} to extend an acronym already used

\acrodef{acl}[ACL]{Access Control List}
\acrodef{api}[API]{Application Programming Interface}
\acrodef{cctv}[CCTV]{Closed Circuit Television}
\acrodef{cpe}[CPE]{Customer Premise Equipment}
\acrodef{dlp}[DLP]{Data Loss/Leakage Prevention}
\acrodef{dpi}[DPI]{Deep Packet Inspection}
\acrodef{ddos}[DDoS]{Distributed Denial of Service}
\acrodef{foss}[FOSS]{Free and Open-Source Software}
\acrodef{ha}[HA]{Hardware Appliance}
\acrodef{ids}[IDS]{Intrusion Detection System}
\acrodef{ilp}[ILP]{Integer Linear Programming}
\acrodef{isp}[ISP]{Internet Service Provider}
\acrodef{ips}[IPS]{Intrusion Prevention System}
\acrodef{mano}[NFV MANO]{NFV Management and Orchestration}
\acrodef{mips}[MIPS]{Millions of Instructions Per Second}
\acrodef{ml}[ML]{Machine Learning}
\acrodef{nat}[NAT]{Network Address Translation}
\acrodef{nf}[NF]{Network Function}
\acrodef{nfv}[NFV]{Network Function Virtualization}
\acrodef{nsc}[NSC]{Network Service Chaining}
\acrodef{of}[OF]{OpenFlow}
\acrodef{pess}[PESS]{Progressive Embedding of Security Services}
\acrodef{pop}[PoP]{Point of Presence}
\acrodef{ps}[PS]{Port Scanner}
\acrodef{qoe}[QoE]{Quality of Experience}
\acrodef{qos}[QoS]{Quality of Service}
\acrodef{sdn}[SDN]{Software-Defined Networking}
\acrodef{sla}[SLA]{Service Level Agreement}
\acrodef{snf}[SNF]{Security Network Function}
\acrodef{tc}[TC]{Traffic Classifier}
\acrodef{tor}[ToR]{Top of Rack}
\acrodef{tsp}[TSP]{Telecommunication Service Provider}
\acrodef{vm}[VM]{Virtual Machine}
\acrodef{vne}[VNE]{Virtual Network Embedding}
\acrodef{vnep}[VNEP]{Virtual Network Embedding Problem}
\acrodef{vnf}[VNF]{Virtual Network Function}
\acrodef{vsnf}[VSNF]{Virtual Security Network Function}
\acrodef{vpn}[VPN]{Virtual Private Network}
\acrodef{wan}[WAN]{Wide Area Network}
\acrodef{waf}[WAF]{Web Application Firewall}



==> application-centric-security/conclusions.tex <==
\subsection{Conclusions}\label{sec:pess-conclusions}
In this paper, we have tackled the problem of the progressive provisioning of security services by means of \acp{vsnf}. The proposed approach, called \ac{pess}, takes into account  security and \ac{qos} requirements of user applications, while ensuring that computing and network resources are accurately utilised. We have discussed the rationale behind our design decisions and presented an \ac{ilp} formulation and a heuristic algorithm that solve the placement problem. Although we have focused our work on security services, the \ac{pess} approach is applicable to more complex scenarios, where heterogeneous network services provided by means of generic \acp{vnf} coexist. 

The evaluation results demonstrate the benefits of \ac{pess} for both users and operators, with savings in resource utilization and in end-to-end latency. We have also shown that the heuristic implementation of the proposed application-aware approach produces near-optimal solutions and scales well in large and dense networks, indicating the potential of \ac{pess} in real-world scenarios.




==> application-centric-security/sdwan-objective-function.tex <==
\subsection{Objective functions for the SD-Branch scenario}\label{sec:sdwan-appendix}
Unlike network operators, whose ultimate goal is the maximization of profit, enterprises usually require low operational expenditures and \ac{qos} guarantees for their network applications. As a result, the enterprise objectives can be formulated for the PESS ILP-based algorithm with an objective function that minimizes the number of active physical nodes, thus reducing the energy consumption. In addition, the \ac{qos} enforcement can be achieved by minimizing the total end-to-end latency of the security service chains. 

\textbf{Energy saving.} Given the physical network $\mathcal{G}$ in a SD-Branch-enabled enterprise, and a security service $\mathcal{G}_s$, find a suitable mapping of $\mathcal{G}_s$ on $\mathcal{G}$, which minimizes the number of active physical nodes of $\mathcal{G}$. 

\begin{equation}\label{eq:energy_objective1}
\min \sum_{i\in N} z_i
\end{equation}

In Eq. (\ref{eq:energy_objective1}), $z_i$ is a binary variable which takes value $1$ if and only if the physical node $i$ is active. $z_i$ is subject to the following constraints:
\begin{fleqn}[2pt]
	\begin{align}
	\begin{split}\label{eq:energy_constraints1}
	\quad &\textstyle \sum_{\{c\in C_s, u\in V^c\}} x^c_{i,u} \leq \mathcal{M}\cdot z_i\quad\forall i\in N
	\end{split}\\[0.5ex]
	\begin{split}\label{eq:energy_constraints2}
	\quad &\textstyle z_i\leq \sum_{\{c\in C_s, u\in V^c\}} x^c_{i,u}\quad\forall i\in N 
	\end{split}
	\end{align}
\end{fleqn}
Constraints (\ref{eq:energy_constraints1}) and (\ref{eq:energy_constraints2}) assure that a physical node is marked as active if at least one \ac{vsnf} is mapped to it. The big-M parameter $\mathcal{M}$ must be set such that $\mathcal{M}>|N|$.

\textbf{Minimum latency.} Given the physical network $\mathcal{G}$ and a security service $\mathcal{G}_s$, find a suitable mapping of $\mathcal{G}_s$ on $\mathcal{G}$, which minimizes the end-to-end latency of the chains of $\mathcal{G}_s$. The goal in this case is to maximize the level of \ac{qos} for all the applications, including common enterprise latency-sensitive applications such as VoIP telephony, video conferencing and CCTV systems.
\begin{equation}\label{eq:energy_objective2}
\min \sum_{c\in C_s}\Big(\pi^c+\sum_{\mathclap{i\in N, u\in V^c}} x^c_{i,u}\cdot \lambda^c_{i,u}+\sum_{\mathclap{\substack{i,j\in N,(k,l)\in E\\(u,v)\in U^c_{pairs}}}}y^c_{k,l,i,j,u,v}\cdot (\lambda_{k,l}+\lambda^c_{k,l,i,j})\Big)
\end{equation}

\noindent Eq. (\ref{eq:energy_objective2}) is derived from Constraint (\ref{eq:const_latency}).

==> application-centric-security/system-security.tex <==
\subsection{Virtualized security framework considerations}\label{sec:system_security}

This work proposes a model for the optimal application of security services within enterprise and service provider networks. By this means, we aim to improve the security of the network. 

However, the security of the system itself should also be considered. While a deep analysis of this is out of scope, we highlight a number of considerations that should be made when deploying a virtualized security framework.

Fundamental to the security of the virtualized system is its deployment on a secure physical and network infrastructure. This includes standard security functions such as identity management, access control, authentication, authorization, and accounting (AAA) to ensure appropriate control and access to the services hosted on the platform.

From the \ac{vnf} perspective, these can be provisioned as virtual machines or containers on the physical nodes. A detailed analysis of the potential security vulnerabilities of \ac{nfv} was presented in \cite{ref_etsinfvsec001}. A range of potential areas of concern were identified, which have subsequently been addressed in individual specification documents. Although work towards solutions to the vulnerabilities is ongoing, the specification documents represent recommendations for the secure implementation of the \ac{vnf} platform.

Current best practices for data centre security include ``micro-segmentation'' to segment the network and apply fine-grained controls/policies to protect applications and workload, and contain the lateral movement of attackers. This is based on a zero-trust policy. This approach complements the veto constraint in the \textit{AA/PESS} algorithm to protect specific functions/applications. 

Finally, as presented in Section \ref{sec:sota}, current solutions to the \ac{VNF} embedding problem generate a new set of service chains based on the solution computation. This introduces the issue of churn with the potential for traffic to be redirected to a different path in the network. The vulnerability of applications to attack during this transition process has not been analysed. In contrast, the implicit design of the \textit{PESS} solution is a progressive embedding that does not require an adjustment to provisioned service chains. This protects these applications from an interruption in security protection.



==> ddos-detection-cnn/background.tex <==
\section{Background}
\subsection{Artificial Neural Networks}
\textit{Introduction to ANNs (with some details related to CNNs and RNNs) and their benefits in anomaly/DDoS detection.}
\subsection{Datasets}\label{sec:datasets}
Our deep learning model has been validated with recent datasets ISCXIDS2012 \cite{ISCXIDS2012}, CICIDS2017 \cite{CICIDS2017} and CSECICIDS2018 \cite{CSECICIDS2018} provided by the Canadian Institute for Cybersecurity of the \ac{unb}, Canada. They consist of several days of network activity, normal and malicious, including \ac{ddos} attacks. The three datasets are publicly available in form traffic traces in \textit{pcap} format including full packet payloads, plus supplementary text files containing the labels and statistical details for each traffic flow. 

The \ac{unb} researchers have generated these datasets by using profiles to accurately represent the abstract properties of human and attack behaviours. One profile characterises the normal network activities and provides distribution models for applications and  protocols (HTTP, SMTP, SSH, IMAP, POP3, and FTP) produced with the analysis of real traffic traces. Other profiles describe a variety of attack scenarios based on recent security reports. They are used to mimic the behaviour of the malicious attackers by means of custom botnets and well-known \ac{ddos} attacking tools such as High Orbit Ion Cannon (HOIC)~\cite{hoic} and its predecessor, the Low Orbit Ion Cannon (LOIC)~\cite{loic}. HOIC and LOIC has been widely used by Anonymous and other hacker groups in some highly-publicized attacks against PayPal, Mastercard, Visa, Amazon, Megaupload, among others.

Table \ref{tab:datasets} shows the parts of the three datasets used in this work. In the table, the column \textit{Traffic trace} specifies the name of the trace, according to \cite{ISCXIDS2012}, \cite{CICIDS2017} and \cite{CSECICIDS2018}. With respect to the original file, the trace \textit{Fri7PM} has been reduced to timeslot 3.30PM-5.00PM to exclude malicious packets related to other cyber attacks (port scans and backdoors). 
However, as this results in a limited number of benign flows for dataset CICIDS2017, flows from trace \textit{Mon3} has been used for balancing without losing precious malicious flows, as described in Section \ref{sec:features}. 

\begin{table}[h!]
	\caption{The datasets used for the evaluation.} 
	\label{tab:datasets}
	\small % text size of table content
	\centering % center the table
	\begin{tabular}{llccc} \toprule[\heavyrulewidth]
		\textbf{Dataset} & \textbf{Traffic trace} & \textbf{\#Flows} & \textbf{\#Benign} & \textbf{\#Attack} \\ \midrule[\heavyrulewidth]
		ISCXIDS2012	& Tue15 & 571698 & 534320 & 37378\\ \midrule
		\multirow{2}*{CICIDS2017}  
		& Mon3 & 529518 & 529518 & 0 \\ 
		& Fri7PM & 225745 & 97718 & 128027 \\ \midrule
		CSECICIDS2018& Wed21 & 1048575 & 360832 & 687743\\ \bottomrule[\heavyrulewidth]
	\end{tabular}
\end{table}


==> ddos-detection-cnn/conclusions.tex <==
\subsection{Conclusions}\label{sec:lucid-conclusions}

%\textit{Future work: evaluation with other types of attacks (DoS, port scans, etc.), evaluation using the dev board with live traffic}

The challenge of \ac{ddos} attacks continues to undermine the availability of networks globally. In this work, we have presented a \ac{dl}-based \ac{ddos} detection architecture. Our design has targeted a practical, lightweight implementation with low processing overhead and attack detection time. The benefit of the \ac{dl} model is to remove threshold configuration as required by statistical detection approaches, and reduce feature engineering and the reliance on human experts required by alternative \ac{ml} techniques. This enables practical deployment. 

In contrast to existing solutions, our unique traffic pre-processing mechanism acknowledges how traffic flows across network devices and is designed to present network traffic to the \ac{dl} model for online \ac{ddos} attack detection. Our evaluation results demonstrate that \ourtool\ matches the existing state-of-the-art performance. However, distinct from existing work, we demonstrate consistent detection results across a range of datasets, demonstrating the stability of our solution. Furthermore, our evaluation on a resource-constrained device demonstrates the suitability of our model for deployment in resource-constrained environments. Specifically, we demonstrate a 40x improvement in processing time over similar state-of-the-art solutions. Finally, we have also presented an activation analysis to explain how \ourtool{} learns to detect \ac{ddos} traffic, which is lacking in existing works. 

%and memory footprint of 40 and 400 times, respectively

%In order to provide a comprehensive, end-to-end presentation of our practical attack detection solution, we have focused this work on \ac{ddos} attack detection. However, as described throughout the paper, \ourtool\ is designed to enable reuse with alternative network data. 

%As future work, we aim to evaluate \ourtool\ with alternative network data such as the detection of other network attacks and to demonstrate live attack detection.  


==> ddos-detection-cnn/detection.tex <==
\section{\ac{cnn}-based algorithm for DDoS detection}\label{sec:detection} 



==> ddos-detection-cnn/features.tex <==
\section{Data pre-processing}\label{sec:features}

The objective of data pre-processing in our system is to shape the input as time-series data as per the convention for real-time, online deployed systems. We ensure the datasets are balanced with equal numbers of malicious and benign flows to reduce bias in the learning process. This gives a greater degree of confidence the deep learning network is learning the correct feature representations from the temporal patterns in the traffic flows.

%The objective of data pre-processing in our system is threefold: (i) allow the neural network to capture the temporal patterns in the traffic flows, (ii) train the neural network with traffic examples that are compatible with online systems, where the input is the traffic collected over fixed or variable time windows,  and (iii) balance the datasets and avoid data skewness. 

\begin{table*}[!t]
	\centering
	\small
	\caption{A TCP flow example before normalization.}
	\label{tab:features}
	\renewcommand{\arraystretch}{1.2}
	\begin{threeparttable}
		%\begin{adjustbox}{width=1\textwidth}
			\begin{tabular}{rc|c|c|c|c|c|c|c|c|c|c|c}
				\Cline{0.8pt}{2-13}
				%\rowcolor{mygray}
				&
				\textbf{Pkt} & \begin{tabular}{@{}c@{}}\textbf{Time}\\\textbf{(sec)}\tnote{1}\end{tabular} & \begin{tabular}{@{}c@{}}\textbf{Pkt}\\\textbf{Len}\end{tabular} & 
				\begin{tabular}{@{}c@{}}\textbf{IP}\\\textbf{Flags}\end{tabular} & \begin{tabular}{@{}c@{}}\textbf{Hdr}\\\textbf{Len}\end{tabular} & \textbf{Protocols}\tnote{2} & \begin{tabular}{@{}c@{}}\textbf{TCP}\\\textbf{Segm. Len}\end{tabular} & \begin{tabular}{@{}c@{}}\textbf{TCP}\\\textbf{Ack}\end{tabular} & \begin{tabular}{@{}c@{}}\textbf{TCP}\\\textbf{Flags}\end{tabular} & \begin{tabular}{@{}c@{}}\textbf{TCP}\\\textbf{WSize}\end{tabular} & \begin{tabular}{@{}c@{}}\textbf{UDP}\\\textbf{Len}\end{tabular} & \begin{tabular}{@{}c@{}}\textbf{ICMP}\\\textbf{Type}\end{tabular}  \\ \Cline{0.8pt}{2-13}
				
				\multirow{5}*{\hspace{-1em}\rotatebox[origin=c]{90}{\textit{Packets}}\vspace{0.5em}$\left\{\begin{matrix}\vspace{5.5em}\end{matrix}\right.$\hspace{-1em}}
				& 0 & 0 & 1078 & 0x4000 & 20 & 0010010001010b & 1024 & 303 & 0x018 & 7504 &  0 & 0 \\ \cline{2-13}
				& 1 & 0.040 & 1514  & 0x4000 & 20 & 0010010001010b & 1460 & 303 & 0x010 & 7504 & 0 & 0 \\ \cline{2-13}
				& \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots \\  \cline{2-13}
				& k & 0.513 &  60  & 0x0000 & 20 & 0010010001000b & 0 & 122485 & 0x010 & 9916 & 0 & 0 \\ \cline{2-13}
				\multirow{4}*{\hspace{-1em}\rotatebox[origin=c]{90}{\textit{Padding}}\hspace{-0.2em}\vspace{0.5em}$\left\{\begin{matrix}\vspace{3.9em}\end{matrix}\right.$\hspace{-1em}} 
				& k+1 & 0 & 0 & 0 & 0 & 0000000000000b & 0 & 0 & 0 & 0 & 0 & 0 \\ \cline{2-13}
				& \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots \\  \cline{2-13}
				& \textit{P} & 0 & 0 & 0 & 0 & 0000000000000b & 0 & 0 & 0 & 0 & 0 & 0 \\ 
				\Cline{0.8pt}{2-13}
			\end{tabular}
		%\end{adjustbox}
		\vspace{0.2em}
		\begin{tablenotes}
			\scriptsize
			\setlength{\itemindent}{0.5em}
			\item[1] Relative time from the first packet of the flow.
			\item[2] Binary representation of the list of protocols recognized in the packet using the well-known \ac{bow} model. It includes protocols from Layer 2 (\textit{arp})
			\item[] to common clear text application layer protocols such as \textit{http}, \textit{telnet}, \textit{ftp} and \textit{dns}. 
		\end{tablenotes}
	\end{threeparttable}	
\end{table*}

As mentioned in Section \ref{sec:datasets}, the \ac{unb} datasets consist in a set of traffic traces in \textit{pcap} format. Initially, the traffic traces are parsed to build a preliminary representation of traffic flows in form of arrays of packet attributes. More precisely, given a time window of length $T$ seconds, each pcap file is parsed starting from the packets with capture time between $t_0$, the capture time of the first packet, and time $t_0+T$ (Figure \ref{fig:pcap-parsing}). 

\begin{figure}[h!]
	\begin{center}
		\includegraphics[width=1\linewidth]{pcap_a}
		\caption{Pcap file parsing.}
		\label{fig:pcap-parsing}
	\end{center}
\end{figure}

From each packet, we extract \features\ attributes (see Table \ref{tab:features}, from \textit{Time} to \textit{ICMP Type}). The attributes of the packets belonging to the same flow are grouped in chronological order to form an array of dimension $[P,F]$, where $F$ is the number of features (\features) and $P$ is the maximum number of packets the parsing process collects for each flow within the time window. Like $T$, $P$ is a hyperparameter for our \ac{dl} models. Flows longer than $P$ are truncated, while shorter flows are zero-padded at the end. The same process is repeated for the packets within time window $[t_0+T,t_0+2T]$ and so on, until the end of the file. This mechanism simulates the capturing process of online systems, where the traffic is collected for a certain amount of time before being process by the anomaly detection algorithms. Hence, such algorithms must base their decisions on portions of traffic flows, without the knowledge of their whole life. 

\begin{figure}[h!]
	\begin{center}
		\includegraphics[width=0.95\linewidth]{pcap_b}
		\caption{New dataset format.}
		\label{fig:dataset-format}
	\end{center}
\end{figure}

Short time windows enable the online systems to detect DDoS attacks within a very short period of time. On the other hand, higher values of $T$ and $P$ guarantee more information on flows to the detection algorithms, resulting in higher detection accuracy. The sensitivity of the proposed \ac{dl} models to the values of $T$ and $P$ is evaluated in Section \ref{sec:evaluation}.     

In the next stage of the data preprocessing, the attributes are normalized and the arrays are zero-padded so that each flow is of fixed length. The resulting new dataset is sketched in Fig. \ref{fig:dataset-format}, where each column is a compact graphical representation of an example. Colored boxes are the packets in form of \features\ normalized attributes (upper part of Table \ref{tab:features}), while the white boxes represent the zero-padding (lower part of the Table). %Labels are collected from the text file provided with each traffic trace and assigned to the examples according to the new dataset format.

As shown in the figure, packets of the same flow may result in multiple examples (e.g., packets from flows $F1$, $F2$, $F3$ and $F4$), exactly how it would happen in an online system where one flow can span multiple time windows. Please note that, the labels assigned to the examples are consistent throughout the dataset, i.e. examples obtained from packets belonging to the same flow receive the same label, according to the label file provided with the original dataset (in Fig. \ref{fig:dataset-format}, all examples with packets from flow $F3$ are labelled as malicious). 

Finally, each dataset is balanced to have approximately the same number of benign and malicious examples. This operation is done by randomly mixing the \ac{ddos} examples with a subset of benign examples. In the case of dataset CICIDS2017, we also used some benign examples from trace \textit{Mon3} (see Table \ref{tab:datasets}) in order to achieve the balancing without the need of discarding \ac{ddos} examples.  

==> ddos-detection-cnn/main.tex <==


\newcommand{\highlightnewtext}{1}
\newcommand{\keepoldtext}{0}

\ifnum\highlightnewtext=1
\newcommand{\revised}[1]{{\leavevmode\color{blue}{NEW: #1}}}
\else
\newcommand{\revised}[1]{{\leavevmode\color{black}{#1}}}
\fi

\ifnum\keepoldtext=1
\newcommand{\original}[1]{{\leavevmode\color{orange}{OLD: #1}}}
\else
\newcommand{\original}[1]{}
\fi

\newcommand{\mytinysize}{\fontsize{6}{7}\selectfont}
\pgfplotsset{
	compat = newest,
	tick label style={font=\sffamily\scriptsize},
	label style={font=\sffamily\scriptsize},
	legend style={font=\sffamily\mytinysize\raggedleft},
	legend cell align=left,
	grid style={dotted,gray}
}

\newcolumntype{?}{!{\vrule width 0.8pt}}

\definecolor{mygray}{RGB}{220,220,220}
\definecolor{skyblue}{RGB}{86,180,233}
\definecolor{bluish-green}{RGB}{0,158,115}
\definecolor{myblue}{RGB}{86,114,178}
\definecolor{vermilion}{RGB}{213,94,0}
\definecolor{reddish-purple}{RGB}{204,121,167}

\newcommand{\features}{11}
\newcommand{\ourtool}[0]{\textsc{Lucid}}

\newlength{\Oldarrayrulewidth}
\newcommand{\Cline}[2]{%
	\noalign{\global\setlength{\Oldarrayrulewidth}{\arrayrulewidth}}%
	\noalign{\global\setlength{\arrayrulewidth}{#1}}\cline{#2}%
	\noalign{\global\setlength{\arrayrulewidth}{\Oldarrayrulewidth}}}

\newcommand*{\rb}[1]{\raisebox{2ex}{\smash{#1}}}

\graphicspath{{artworks/}}
\DeclareGraphicsExtensions{.pdf,.jpeg,.png}


\begin{abstract}
\ac{ddos} attacks are one of the most harmful threats in today's Internet, disrupting the availability of essential services. The challenge of \ac{ddos} detection is the combination of attack approaches coupled with the volume of live traffic to be analysed. In this paper, we present a practical, lightweight deep learning \ac{ddos} detection system called \ourtool, which exploits the properties of \acp{cnn} to classify traffic flows as either malicious or benign. We make four main contributions; (1) an innovative application of a \ac{cnn} to detect \ac{ddos} traffic with low processing overhead, (2) a dataset-agnostic pre-processing mechanism to produce traffic observations for online attack detection, (3) an activation analysis to explain \ourtool{}'s \ac{ddos} classification, and (4) an empirical validation of the solution on a resource-constrained hardware platform. Using the latest datasets, \ourtool\ matches existing state-of-the-art detection accuracy whilst presenting a 40x reduction in processing time, as compared to the state-of-the-art. With our evaluation results, we prove that the proposed approach is suitable for effective \ac{ddos} detection in resource-constrained operational environments. 
\end{abstract}


\input{acronyms}
\input{introduction}
\input{related}
\input{methodology}
\input{setup}
\input{evaluation}
\input{analysis}
\input{usecase}
\input{conclusions}

